Architecture for Health Initiative (Arch4Health): Computational Challenges in Health-Related Applications and the Role of Computer Architecture in Addressing Them

Recent biotechnological advances enable high-throughput, low-cost, and accurate biological data generation. This wealth of data enables unique opportunities for advancing healthcare. Despite these opportunities, efficiently analyzing large-scale biological data poses significant challenges for conventional computing systems. These systems often cannot keep up with the high-throughput rate at which data is generated, and they face additional constraints related to energy efficiency, scalability, privacy, and security. Therefore, to facilitate the wide adoption of recent advances in healthcare, there is a need to optimize the computing systems to enable high-performance, energy-efficient, low-cost, private, and secure analysis of biological data. We introduce the Architecture for Health (Arch4Health) initiative, which aims to (i) identify and analyze key computational challenges in current and future health- and life science-related applications and (ii) explore how computer architects and computing system designers can advance healthcare by addressing these challenges. In this short paper, we first present the motivations behind the Arch4Health initiative and, second, elaborate on its vision and goals, related topics, Arch4Health workshops, and future outlooks.

==> _archive/commands_taps.tex <==
\newcommand{\citegraphacc}{gihawi2023major,pockrandt2022metagenomic,berger2023navigating,meyer2021critical,alser2020technology,alser2022molecules}

\newcommand{\citesbs}{bentley_accurate_2008,turcatti_new_2008,fuller_method_2011}

\newcommand{\citesmrt}{eid_real-time_2009}

\newcommand{\citenanopore}{laszlo_decoding_2014,deamer_three_2016,zhang_single-molecule_2024}

\newcommand{\citesequencing}{\citesbs,\citesmrt,\citenanopore,stoler2021sequencing,davis2021sequencerr,sereika2022oxford,ni2023benchmarking}

\newcommand{\citepersonalized}{branco_bioinformatics_2021,quazi_artificial_2022,papadopoulou_application_2023,tafazoli_applying_2021,moon_precision_2022,hussen_emerging_2022,russell_pharmacogenomics_2021,verma_nanopore_2024,sweeney2021rapid}

\newcommand{\citeoutbreakrapid}{dunn_squigglefilter_2021,comin_investigation_2020,Quick2016}

\newcommand{\citeoutbreak}{\citeoutbreakrapid,li_application_2021,deng_integrated_2021,bloom2021massively,yelagandula2021multiplexed}

\newcommand{\citeagriculture}{campos_high_2021,gao_genome_2021,van_dijk_machine_2021,sun_twenty_2022,thudi_genomic_2021,shen_omics-based_2022,shahroodi_demeter_2022,prasad2021soil,Mascher2024,Schreiber2024}

\newcommand{\citeevolution}{kanzi_next_2020, wang_population_2020, Prohaska2019human, kanehisa_toward_2019, signor_evolution_2018, coolon_tempo_2014, wittkopp_cis-regulatory_2012, fay_evaluating_2008, whitehead_variation_2006, wray_evolution_2003}

\newcommand{\citecancer}{jia_high-throughput_2022,liu_mrna-based_2023,van_de_sande_applications_2023,chakravarty_clinical_2021,cortes-ciriano_computational_2022,deveson_evaluating_2021,xiao_toward_2021,szustakowski_advancing_2021,lei_applications_2021,han_single-cell_2022,stadler_therapeutic_2021,tan_targeted_2022,degasperi_substitution_2022,xu_single-cell_2022,horak_comprehensive_2021,waarts_targeting_2022,xiao_tumor_2021,nandwani_lncrnas_2021,marchetti_error-corrected_2023,chen_next-generation_2021}

\newcommand{\citemetagenomicsegs}{danko2021global,paoli2022biosynthetic,edgar2022petabase,prasad2021soil,biodigs2026,Ryon2022,Zhu2025}

\newcommand{\citemgprecision}{mousa2024gut,tegegne2025g,zhao2024application}

\newcommand{\citemgurgentclinical}{sweeney2021rapid,gu2021rapid,charalampous2024routine,Heitz2023,Alcolea-Medina2025,LIANG2023101898,Chien2022,Neyton2023,GENG202181,Ren2021}

\newcommand{\citemgbiodiversity}{danko2021global,biodigs2026,Zhu2025}

\newcommand{\citemgcommunicable}{john2021next,nagy2021targeted,downie2023surveillance}

\newcommand{\citemgtracing}{hadfield2018nextstrain,parkins2024wastewater,cdcpulsenet}

\newcommand{\citealgoptimization}{li2018minimap2,marco2021fast,marcosola2023optimal,grootkoerkamp2024apa2,sadasivan2024genomic,tseng2025ultrafast,walia2025ultrafast,kim_fastremap_2022,Ashyralyyev2026gencore,ashyralyyev2026lcpan,alicioglu2024pairwise,manber1993suffix}

\newcommand{\citemgalgoptimization}{song2024centrifuger,pockrandt2022metagenomic,song2024centrifuger,Fan2021}

\newcommand{\citegraphalgoptimization}{siren2021pangenomics,Chandra2023,Ivanov2022,Ma2023,Hwang2025MEMO,Romain2023svjedi}

\newcommand{\citehwoptimization}{doblas2025smx,mutlu2023accelerating,alser2022molecules,shahroodi2023swordfish,subramaniyan2021accelerated,khatamifard2021genvom,li2021pim,turakhia2018darwin,chen2021high,haghi2021fpga,li2021pipebsw,ham2021accelerating,cali2020genasm,Zhang_2023_alignerD,soysal2025mars,kim2018grim,mao2022genpip,dphls2026,Walia2024talco,sadasivan2024genomic,Turakhia2025toward,Turakhia2019darwinwga,simon2026processing,eudine2026genpairx,Lindegger2023scrooge}

\newcommand{\citemghwoptimization}{kobus2021metacache,wang2023gpmeta,zhang2023genomix,cervi2022metagenomic,wu2021sieve,shahroodi2022krakenonmem,shahroodi2022demeter,dashcam23micro,hanhan2022edam,zou2022biohd,dunn2021,shih2023efficient}

\newcommand{\citegraphhwoptimization}{cali2022segram,Zhang2024Harp,Zeng2024asgdp,Shen2024128parallel,Li2024,Awan2021,Feng2021,Zhang2025,kim2025nmp,Huang2023meg2,Zhou2021,Sarkar2021,Galanos2021,Sinha2022,Chen2023}

\newcommand{\citefilteroptimizationadditional}{singh2021fpga,hameed2021alpha,guo2019hardware}

\newcommand{\citegenomiccompression}{cogo2021genodedup,kokot2022colord,Meng2023,dufort2021renano,dragenora,yang2025gpufastqlz,chen2023efficient,lan2021genozip}

\newcommand{\citemapping}{ angizi2020pim, fujiki2020seedex, ham2020genesis, kaplan2020bioseal, zeni2020logan, ahmed2019gasal2, angizi2019aligns, gupta2019rapid, wu2019fpga, banerjee2018asap, cheng2018bitmapper2, fei2018fpgasw, fujiki2018genax, houtgast2018hardware, huangfu2018radar, rucci2018swifold, zokaee2018aligner, goyal2017ultra, houtgast2017efficient, nishimura2017accelerating, chen2016spark, de2016cudalign, xin2016optimal, chen2015novel, liu2015gswabe, waidyasooriya2015hardware, wilton2015arioc, xin2015shifted, chen2014accelerating, madhavan2014race, liu2013cudasw++, xin2013accelerating}

\newcommand{\citeasm}{cali2020genasm,alser2017gatekeeper,alser2017magnet,alser2019shouji,alser2020sneakysnake,kim2018grim,kim2019airlift,kim2024airlifttcbb,needleman1970general,smith1981identification,gotoh1982improved}

\newcommand{\citegc}{cai2017error,kim2023decoupled,cai-insidessd-2018}

\newcommand{\citewearleveling}{chang2007efficient,cai2017error,cai-insidessd-2018}

\newcommand{\citeflashrefresh}{cai2013error,luo2018improving, cai2017error,cai2012flash,
cai-hpca-2017,luo-hpca-2018,cai2015read, ha2015integrated, cai-insidessd-2018,luo2015warm}

\newcommand{\citebasecalling}{cock2009sanger,alser2022molecules,lou2020helix,shahroodi2023swordfish,Samarakoon2023accelerated}

\newcommand{\citebasecallnanodnn}{cavlak2022targetcall,cavlak_targetcall_2024,xu2021fast,peresini_nanopore_2021,oxford_nanopore_technologies_dorado_2024,singh_rubicon_2024,xu_lokatt_2023,konishi_halcyon_2021,yeh_msrcall_2022,noordijk_baseless_2023,huang_sacall_2022}

\newcommand{\citebasecallnanohmm}{loman_complete_2015,david_nanocall_2017,schreiber_analysis_2015}

\newcommand{\citehwmapping}{alser2020accelerating,cali2020genasm,turakhia2018darwin,khatamifard2021genvom,li2021pim,chen2021high,haghi2021fpga,li2021pipebsw,ham2021accelerating,doblas2025smx,kim2018grim,alser2020sneakysnake,bingol2021gatekeeper,mao2022genpip,mansouri2022genstore,alser2017gatekeeper,alser2019shouji,alser2017magnet,Zhang_2023_alignerD,cali2022segram,mutlu2023accelerating,alser2022molecules,subramaniyan2021accelerated,fujiki2018genax,fujiki2020seedex,zeni2020logan,ahmed2019gasal2}

\newcommand{\citevariantcallers}{mandiracioglu_ecole_2024,smolka_detection_2024,lin_svision_2022,popic_cue_2023,zheng_symphonizing_2022,ahsan_nanocaller_2021,minoche_clinsv_2021,zheng_svsearcher_2023,alser2022molecules,Olson2023,Park2025,dunn2023n}

\newcommand{\citeassembly}{Haghshenas2020, nurk_hicanu_2020, ruan_fast_2020, shafin_nanopore_2020, kolmogorov_assembly_2019, Zimin2017hybrid, kamath_hinge_2017, koren_canu_2017, xiao_mecat_2017, chin_phased_2016, lin_assembly_2016, iqbal_novo_2012, butler_allpaths_2008, myers_fragment_2005, myers_whole-genome_2000, bonfield_new_1995, fleischmann_whole-genome_1995, kececioglu_combinatorial_1995, peltola_seqaid_1984}

\newcommand{\citetaxclassification}{wu2021sieve,song2024centrifuger,Fan2021,pockrandt2022metagenomic,lemane2023kmindex,shen2022kmcp,sun2021challenges,dimopoulos2022haystac,meyer2021critical}

\newcommand{\citemappairalign}{marco-sola_fast_2021,Lindegger2023scrooge,marco-sola_optimal_2023,needleman_general_1970,smith_identification_1981,senol_cali_genasm_2020,waterman_biological_1976,gotoh_improved_1982,wagner_string--string_1974,sankoff_matching_1972,groot_koerkamp_exact_2024,sellers_theory_1974,ukkonen_algorithms_1985}

\newcommand{\citesscaiml}{lee2025aif,li2023ecssd,Adnan2024,Peng2025xharvest,Tang2024transformerisp,lee2022smartsage,wang2024beacongnn,jang2024smart,Chen2025reis,Yu2024cambriconllm,Niu2024flashgnn,Kim2023optimstore,Sun2025lincoln,Taranco2025iris,Pan2025instattention,Mahapatra2025isp_rag}

\newcommand{\citesscgraphs}{jun2018grafboost,xu2019vstore,matam2019graphssd}

\newcommand{\citesscotherapps}{lim2021lsm,li2021glist,kang2021s,han2021flash,wang2022memcore,Duffy2023dotori,Park2025anykey,Chen2024aresflash,Wong2025anvil,mahapatra2024instoragedomainspecificaccelerationserverless}

\newcommand{\citegpisp}{wang2019project,kang2021iceclave,zou2022assasin}

\newcommand{\citegpifp}{chun2022pif,chen2024search}

\newcommand{\citegpufp}{chun2024rif,gao2021parabit,park2022flash}

\newcommand{\citegpispfpga}{lee2020smartssd,ajdari2019cidr,Jeong2025upp}

\newcommand{\citegpispgpu}{cho2013xsd}

\newcommand{\citenongenomegraphisp}{matam2019graphssd,Wang2024ndsearch,lee2022smartsage,Niu2024flashgnn,Lee2024presto,Khadirsharbiyani2024smartgraph,Zhang2025taijigraph,An2023baraddur,Kang2024sting}

\newcommand{\citenongraphgenomeisp}{mansouri2022genstore,abakus23taco,megis,kim2025nmp,soysal2025mars,zheng2025storage}

\newcommand{\citedp}{alser2020accelerating,alser2017gatekeeper,alser2017magnet,alser2019shouji,alser2020technology,cali2020genasm,kim2018grim,needleman1970general,smith1981identification,alser2020sneakysnake}

\newcommand{\citeflash}{cai-insidessd-2018,cho2024aero,nadig2026conduit,nadig2023venice,park2022flash,park-asplos-2021,kim2021performance}

\newcommand{\citebasecallsbs}{cacho_base-calling_2018,wang_adaptive_2017,ye_blindcall_2014,das_base_2013,renaud_freeibis_2013,das_onlinecall_2012}

\newcommand{\citesignalanalysis}{Bao2021Squigglenet,kovaka_targeted_2021,senanayake_deepselectnet_2023,sam_kovaka_uncalled4_2024,lindegger_rawalign_2024,firtina2023rawhash,firtina2023rawhash2,firtina_rawsamble_2024,shih_efficient_2023,sadasivan_rapid_2023,dunn_squigglefilter_2021,shivakumar_sigmoni_2024,sadasivan_accelerated_2024,samarasinghe_energy_2021}

\newcommand{\citesinglecell}{wen2022singlecell,ni2023benchmarking,jia_high-throughput_2022,van_de_sande_applications_2023,lei_applications_2021,han_single-cell_2022,xu_single-cell_2022}

\newcommand{\citetranscriptomics}{chen2023hitchhikers,Sibbesen2023,haas_forensic_2021,clough2023ncbigeo}

\newcommand{\citeauditandprivacy}{Pattengale2020Decentralized,ma2020efficient,bonomi2020privacy}

\newcommand{\citeerrorcorrection}{firtina_hercules_2018,stanojevic_telomere--telomere_2024,kang_hybrid-hybrid_2023,holley_ratatosk_2021,zhu_lcat_2023}

\newcommand{\citepum}{ xi2020memory, angizi2019dna, angizi2019graphide, seshadri2019dram, slesazeck20192tnc, angizi2018cmp, angizi2018pima, eckert2018neural, yu2018memristive, aga2017compute, bhattacharjee2017revamp, hamdioui2017myth, seshadri2017ambit, Shafiee2016, chang2016low, gaillardon2016plim, seshadri2016buddy, seshadri2016processing, zheng2016tcam, hamdioui2015memristor, seshadri2015fast, xie2015fast, kang2014energy, seshadri2013rowclone}
